PageRank computation for Higher-Order Networks

Higher-order networks are efficient representations of sequential data. Unlike the classic first-order network approach, they capture indirect dependencies between items composing the input sequences by the use of \textit{memory-nodes}. We focus in this study on the variable-order network model introduced in [Xu et al. (2016);Saebi et al. (2020)]. Authors suggested that random-walk-based mining tools can be directly applied to these networks. We discuss the case of the PageRank measure. We show the existence of a bias due to the distribution of the number of representations of the items. We propose an adaptation of the PageRank model in order to correct it. Application on real-world data shows important differences in the achieved rankings. \keywords{Higher-order Networks, Sequential data, Random walks, PageRank

==> DB1B/topPRDB1B.tex <==
\begin{table}[h!]
\centering
\caption{
    %\red{Ordre correct pour les col: K1, K1 biaisé, K von, K von U (corrigé)} 
    Airports' tops 10 PageRank.}
\label{tab:top10_airports}
\resizebox{1.\textwidth}{!}{\begin{tabular}{|l|lcc|lcc|lcc|lcc|}
\cline{2-13}
\multicolumn{1}{l|}{}  & \multicolumn{3}{c|}{$\frank$} & \multicolumn{3}{c|}{$\brank$} & \multicolumn{3}{c|}{$\hrank$} & \multicolumn{3}{c|}{$\urank$}\\
\cline{1-13}
Rank & Airport ~& $\reprank$ ~& $\vrank$~ & Airport ~& $\reprank$ ~& $\vrank$ & Airport ~& $\reprank$ ~& $\vrank$~ & Airport ~& $\reprank$ ~& $\vrank$\\
\cline{1-13}
1&ATL (GA)&1&1~&ATL (GA)&1&1&ATL (GA)&1&1~&DEN (CO)&5&3\\
2&DEN (CO)&5&3~&ORD (IL)&2&2&ORD (IL)&2&2~&ATL (GA)&1&1\\
3&ORD (IL)&2&2~&DEN (CO)&5&3&DFW (TX)&4&4~&ORD (IL)&2&2\\
4&DFW (TX)&4&4~&DFW (TX)&4&4&DEN (CO)&5&3~&DFW (TX)&4&4\\
5&CLT (NC)&3&5~&CLT (NC)&3&5&CLT (NC)&3&5~&MSP (MN)&8&9\\
6&MSP (MN)&8&9~&PHX (AZ)&9&6&DTW (MI)&6&10~&CLT (NC)&3&5\\
7&PHX (AZ)&9&6~&LAX (CA)&11&7&MSP (MN)&8&9~&SEA (WA)&17&15\\
8&LAX (CA)&11&7~&IAH (TX)&7&8&IAH (TX)&7&8~&DTW (MI)&6&10\\
9&IAH (TX)&7&8~&DTW (MI)&6&10&PHX (AZ)&9&6~&IAH (TX)&7&8\\
10&DTW (MI)&6&10~&MSP (MN)&8&9&LAX (CA)&11&7~&PHX (AZ)&9&6\\
\cline{1-13}
\end{tabular}
}
\end{table}


==> Porto_Taxis/topPRtaxis.tex <==
\begin{table}
\centering
\caption{\tbd{Replace this table with a colored map of Porto city. For each place of interest, we can color them according to its Rank or PR score. Only places which belongs to a top 10 will be labeled in this figure.} Tops 10 PageRank according to HON, Unbiased HON, 1stON and Biased 1stON PR models applied on Porto Taxis data set.}

\label{tab:top10Taxis}
\resizebox{\textwidth}{!}{\begin{tabular}{|l|ccc|ccc|}
\cline{2-7}
\multicolumn{1}{l|}{} & \multicolumn{3}{c|}{$\hrank$} & \multicolumn{3}{c|}{$\urank$}\\
\cline{1-7}
Rank ~& Police Station ~& $\reprank$ ~& $\vrank$ ~& Police Station ~& $\reprank$ ~& $\vrank$ \\
\cline{1-7}
1&None&2&2~&None&3&7\\
2&Polícia de Segurança Pública - 7ª Esquadra&1&1~&None&2&2\\
3&18ª Esquadra da Polícia de Segurança Pública&5&4~&PSP Sra da Hora&10&8\\
4&None&3&7~&18ª Esquadra da Polícia de Segurança Pública&5&4\\
5&PSP Sra da Hora&10&8~&Polícia de Segurança Pública - 7ª Esquadra&1&1\\
6&Polícia de Segurança Pública&6&3~&Polícia de Segurança Pública&6&3\\
7&Polícia: Comando Metr. Porto&8&5~&PSP Maia&11&12\\
8&Policia PSP 13ª&4&6~&Polícia: Comando Metr. Porto&8&5\\
9&Polícia de Segurança Pública&7&10~&Polícia de Segurança Pública&7&10\\
10&PSP Maia&11&12~&Policia PSP 13ª&4&6\\
\cline{1-7}
\multicolumn{1}{l|}{} & \multicolumn{3}{c|}{$\frank$} & \multicolumn{3}{c|}{$\brank$}\\
\cline{1-7}
Rank ~& Police Station ~& $\reprank$ ~& $\vrank$ ~& Police Station ~& $\reprank$ ~& $\vrank$ \\
\cline{1-7}
1&None&2&2~&None&2&2\\
2&18ª Esquadra da Polícia de Segurança Pública&5&4~&Polícia de Segurança Pública - 7ª Esquadra&1&1\\
3&Polícia de Segurança Pública - 7ª Esquadra&1&1~&18ª Esquadra da Polícia de Segurança Pública&5&4\\
4&None&3&7~&Policia PSP 13ª&4&6\\
5&PSP Sra da Hora&10&8~&None&3&7\\
6&Quartel da GNR - GIPS&28&32~&Polícia: Comando Metr. Porto&8&5\\
7&Polícia: Comando Metr. Porto&8&5~&PSP Sra da Hora&10&8\\
8&Policia PSP 13ª&4&6~&Polícia de Segurança Pública&6&3\\
9&Polícia de Segurança Pública&6&3~&Polícia de Segurança Pública&7&10\\
10&None&35&34~&None&9&9\\
\cline{1-7}
\end{tabular}
}
\end{table}


==> figs/ex_1on.tex <==
\begin{tikzpicture}[scale = 1.]
\node[draw,scale=1.,circle] (X) at (0,-1) {$x$};
\node[draw,scale=1.,circle] (Y) at (0,1) {$y$};
\node[draw,scale=1.,circle] (A) at (0,0) {$a$};
\node[draw,scale=1.,circle] (C) at (1,0) {$c$};
\node[draw,scale=1.,circle] (B) at (2,0)  {$b$};

\draw[->,>=latex, line width=1.5pt] (X)--(A);
\draw[->,>=latex, line width=1.5pt] (Y)--(A);
\draw[->,>=latex, line width=1.5pt] (A) to [bend right=15] (C);
\draw[->,>=latex, line width=1.pt] (C) to [bend right=10] (A);
\draw[->,>=latex, line width=1.5pt] (B) to [bend right=15] (C);
\draw[->,>=latex, line width=1.pt] (C) to [bend right=10] (B);
\end{tikzpicture}
